Social Media-based User Embedding: A Literature Review

Automated representation learning is behind many recent success stories in machine learning. It is often used to transfer knowledge learned from a large dataset (e.g., raw text) to tasks for which only a small number of training examples are available. In this paper, we review recent advance in learning to represent social media users in low-dimensional embeddings. The technology is critical for creating high performance social media-based human traits and behavior models since the ground truth for assessing latent human traits and behavior is often expensive to acquire at a large scale. In this survey, we review typical methods for learning a unified user embeddings from heterogeneous user data (e.g., combines social media texts with images to learn a unified user representation). Finally we point out some current issues and future directions.

==> prediction.tex <==
\section{Prediction}

\section{Overview of Studies}
\begin{table*}[ht!]
\small
\centering
    \caption{Summary of Studies}
    \label{tab:overview}
    \begin{tabular}{@{}p{4.1cm}p{3.5cm}p{4.5cm}p{1cm}p{3cm}@{}}
      \toprule
       \textbf{Paper} & \textbf{Platform} &\textbf{Source Data Type} & \textbf{Size}  & \textbf{Predicted Target}  \\
       \midrule
       %\cite{mislove2010you} & 
       \cite{pennacchiotti2011machine} & Twitter& tweet, user profile & 10,338 & political leaning \\
                                                                       &&& 6,000 &  ethnicity\\
                                                                       &&& 10,000 & user preference \\\hline %starbucks fan
       %\cite{yin2011structural} & Twitter & social network&979 &link prediction \\\hline
       %\cite{mahmud2012tweet} & Twitter & tweet& 9,551 & home location \\\hline short paper
       %\cite{farnadi2013recognising} & Facebook & status, social network & 250 & personality \\\hline % time-related features, other features, short paper
        %\cite{de2013predicting} & Twitter &post, social network, user profile &476& depression \\\hline % engagement, Egocentric Social Graph, emotion, Linguistics
       %\cite{zhang2013predicting} & Facebook& like & 13,619 & purchase behavior \\\hline
       %\cite{mcgee2013location} & &&&location \\\hline
       %\cite{hong2013co} & Twitter & tweet, social network & 765,385 & interests \\\hline
       \cite{kosinski2013private} &Facebook&likes&58,000&age, gender,personality\\
                                                 &&& 46,027 &relationship\\
                                                 &&& 1,200 &substance use\\
                                                 &&& 18,833& religion \\
                                                 &&&  9,752&political leaning\\\hline
       \cite{schwartz2013personality} &Facebook&post & 75,000& age,gender,personality \\\hline
       %\cite{sap2014developing} & Facebook & status & 75,394 & age, gender \\\hline %MyPersonality
       %\cite{yang2015using} & Twitter & tweet & 10,000 & brand preference \\\hline 
      \cite{gao2014modeling} &Twitter&tweet, retweet&&attitude\\
      &&&5,387& (Topic:Fracking)\\
      &&&2,593& (Topic:Vaccination)\\\hline
      \cite{perozzi2014deepwalk} & BlogCatelog & social network & 10,312 & topic categorization\\
      & Flickr & & 80,513 & node classification \\
      & YouTube && 1,138,499 & node classification \\\hline
       %\cite{youyou2015computer} &Facebook& like &70,520 & personality \\\hline
       \cite{preoctiuc2015analysis} & Twitter & tweet,user profile & 5,191 &  occupation\\\hline
       \cite{song2015interest} & Twitter,Facebook,Quora & post, bio description & 1,607 & interest\\\hline 
      % &Facebook & & &  \\ 
       %&Quora&&&\\\hline 
       \cite{hu2016language}&Twitter&tweet&9,800&occupation\\\hline
       \cite{song2016volunteerism} &Twitter,Facebook,Linkedin&tweet, social network &5,436 &volunteerism\\\hline
                   
       \cite{benton2016learning}&Twitter&tweet,social network& 102,328 & topic engagement \\
       												&&&500&friend recommendation\\
                                                    &&&383 & age, gender \\
                                                    &&&396 & political leaning\\\hline % nsupervised  102,328
       %\cite{mahmud2016predicting}&Twitter&tweet& $<1000$ & attitude and actions to brands \\\hline
       \cite{wallace2016modelling} & Twitter & tweets & 12,500 & sarcasm detection  \\\hline
       \cite{ding2017multi} & Facebook & status, like & 1,200 & substance use\\ \hline
         \cite{preoctiuc2017beyond} &Twitter& tweet& 3,938& political leaning \\\hline
         \cite{miura2017unifying} & Twitter & tweet,metadata,network & 279,000& geolocation prediction \\\hline
         \cite{hasanuzzaman2017temporal} & Twitter & tweet & 5,191 & income \\\hline
         %\cite{xu2017embedding} & BlogCateglog & 
         %                       & Flickr & 
         %\cite{singh2017toward}&Instagram & caption, comments, image&699& cyberbullying\\\hline
         \cite{amir2017quantifying}&Twitter& tweets&327&depression \\
         &&& 246 & stress disorder \\\hline
         \cite{liao2018attributed} &Facebook & social network & 17,000+ & link prediction \\
         & DBLP &citation network  & 29,000 & node classification \\
         & Citeseer &citation netowrk & 60,000 & \\\hline
         \cite{zhang2017user} & Google+ & social network & 1206 & node classification, clustering\\
         & Facebook & social network & 755 & \\
            && &  2188 & \\% 
            && &  4145 & \\\hline
         \cite{farnadi2018user} & Facebook & status update, profile picture, likes&5,670 & age, gender, personality\\\hline
         %\cite{fan2018automatic} & Twitter & & & opioid user detection\\\hline
         \cite{zhang2018user} & Flickr & photo, description & 128 & image popularity \\\hline
         \cite{ribeiro2018characterizing} & Twitter &tweet, retweet network & 4,972 & hateful user detection \\\hline
         \cite{zhang2018anrl} & Facebook & social network, attributes & 4,039 & link prediction, node classification\\
                               &           &    & 18,163 &\\
                                 &           &      & 23,377 \\
                                & Citeseer & citation network & 3,312 \\
      \bottomrule
    \end{tabular}
\end{table*} 


In this section, we discuss some methods used in prediction with social media. 

Regression is a form of predictive modeling technique which investigates the relationship between a dependent and one or more independent variable. The regression indicates the significant relationships between dependent variable and independent variable, and the strength of impact of multiple independent variable on a dependent variable. These benefits allow us get insight into human traits and behaviors and help us to evaluate the best set of variables to be used for building predictive models. 

%Classification is a class of algorithms identifying the new observation belong to which categories based on the training data with known categorical information. Some other classical methods widely used include decision tree, naive bayes, SVM, KNN, and logistic regression.

\textbf{Decision tree}: Decision tree is an algorithm having a tree structure and the decision or prediction result is made after traversing from root node to leaf. The learning process involves splitting the raw dataset into subsets based on attribute value test recursively until the dataset has same attribute value. The advantage is the simplicity of explanation and understanding since it is a totally white box model. On the other hand, the overfitting, instability and inaccuracy caused by small change or noise of dataset will be concerns comparing to other methods.

\textbf{Naive Bayes}: Naive Bayes is a probabilistic classifier based on Bayes' theorem. The 'naive' term refers to assumption of independence between each feature regardless of any correlations. Based upon the priori probability of the event, Bayes classifier calculates the posterior probability of each class and select the result with highest one. The training process normally apply the Maximum Likelihood Estimation(MLE) to tune the parameters within the model according to the sampled data. The advantages are high scalability and linear training time rather than expensive iterative approaching approximation method. The disadvantage is lack of concerning the correlation between features which may cause inaccuracy.

\textbf{Logistical Regression}: Logistical Regression is a regression method which model the one or more independent variables into outcome measured with a dichotomous variable. The goal is to explore the relationship between dichotomous characteristics and independent variables using the logistic function.

\textbf{SVM}: Supporting Vector Machine(SVM) is a model generating non-probabilistic binary linear classification outcome based on labeled training data. The main idea is to maximize the gap between groups of points with different categories and test data point will classified based on falling into different sides of gaps.

\textbf{k-NN}: k-Nearest-Neighbors is a method which the object's classification is determined by the majority of k nearest neighbors around based on the euclidean distances. k is an integer normally greater than 1. Besides classification it can also be applied to regression which the outcome value is the average of k nearest neighbors.  


%Generally, most studies will extract data from various sources such as text, pictures, demographic information etc. and produce a feature representation. The researchers will apply the features to smaller labeled dataset to predict different individual characteristics. 

%This survey performs a comprehensive analysis of state-of-the-art methods to model users and predict different individual characteristics using different sources of data in social media.

%Table \ref{tab:overview} shows the overview of these papers. These studies focus on four social media platform: Facebook, Twitter, Reddit and Instagram. 


%\cite{pennacchiotti2011machine} accuracy 2-way political classification
%\cite{mahmud2012tweet} location, recall,classification
%\cite{farnadi2013recognising} We compare the performance of 3 learning algorithms
%trained on these features, namely Support Vector Machine
%with a linear kernel (SVM), Nearest Neighbor with k=1
%(kNN) and Naive Bayes (NB). Personality classification

%\cite{de2013predicting}  Support Vector Machine classifier with a radial-basis
%function (RBF) kernel (Duda et al., 2000). depression 72\%
%\cite{zhang2013predicting} Support Vector Machine classifier, Naive Bayes (NB), LR(best) Overall, the results suggest that SVM and Logistic Regression
%make a much better use of the social features than
%Mapping and Naive Bayes. purchase behavior. 
%\cite{o2013using} Vote: political users 82\% non-political users 62\%
%\cite{youyou2015computer} personality correlation
%\cite{schwartz2013personality} We use a linear support vector machine (SVM) [92] for
%classifying the binary variable of gender, and ridge regression
%[93] for predicting age and each factor of personality.
%\cite{chen2014understanding}The R2 of the linear regressions were small but substantial across all five value dimensions

%Bayesian nonparametric framework of Gaussian Processes (Rasmussen and Williams, 2006), which also accommodates feature interpretation via the Automatic Relevance Determination. This allows us to get insight into differences in language use across job classes and, finally, assess our original hypothesis about the thematic divergence across them. 9 way classification. 
%Classification with Gaussian Processes.  we used the powerful, non-linear GP framework that combines strong predictive performance with feature interpretability Results show that we can achieve a good predictive accuracy, highlighting that the occupation of a user influences text use. 

%\cite{hu2016language} Words and phrases related features have the best performance among the three single type features. This is because words and phrases are the most informative type of features among three. They cover all the terms used in tweets with the cost of high dimensions of features.

%\cite{liu2016analyzing} We use linear regression with Elastic Net regularization (Zou and Hastie 2005) as our prediction algorithm

%\cite{vedula2017emotional} We subsequently construct a binary classifier using the above identified feature set. We use the Gradient Boosted Decision Trees classifier [11] along with 5-fold cross validation on the full dataset of 150 users. The features distinguishing between the users of the two classes in decreasing order of importance are: words expressing negative emotion, self and group-focused pronouns, user clustering coefficient, activity, retweets, mentions and location entropy. We measure the performance of the classifier using the standard metrics of accuracy of both classes, micro-F1 score and macro F1-score. We achieve an accuracy of 0.9 for the depressed class users, a slightly lower accuracy of 0.87 for the normal/non-depressed class of users, a micro-F1 score of 0.9 and a macro-F1 score of 0.8901. Drilling down on the results, we find that only 5 depressed users are misclassified as normal. Of the misclassified normal users, we find that while their tweets do not express depression, they still exhibit an increasing use of words with negative emotions such as violence or anger

%\cite{preoctiuc2017beyond} between conservatives and liberals across various levels of political engagement in D1 and between the two polarized groups in D2. We use logistic regression classification to compare three setups in Table 2 with results measured with ROC AUC

%Schwartz et al., 2013; r = 0.84
%for age and 91.9\% accuracy for gender

%Guassian Process, Support Vector Regression, Linear regression, 
%Classification method: 


%Lexicon creation \cite{sap2014developing} Age and gender are predicted using text-based models described in [32]. These models were trained on data from over 70,000 Facebook users and reports an accuracy of 91.9\% for gender (88.9\% on Twitter data) and Pearson correlation r = 0.84 for age prediction. We derive predictive lexica (words and weights) for age and gender using regression and classification models from word usage in Facebook, blog, and Twitter data with associated demographic labels. The lexica, made publicly available,1 achieved state-of-the-art accuracy in language based age and gender prediction over Facebook and Twitter, and were evaluated for generalization across social media genres as well as in limited message situations. The lexica, in the form of words with associated weights, are derived from a penalized linear regression (for continuous valued age) and support vector classification (for binary-valued gender). In this modality, the lexica are simply a transparent and portable means for distributing predictive models based on words.

%\cite{youyou2015computer} lasso We used LASSO (Least Absolute Shrinkage and Selection Operator) linear regressions (16) with 10-fold cross-validations, so that judgments for each participant were made using models developed on a different subsample of participants and their Likes. 
